Multi-wavelength continuum sizes of protoplanetary discs: scaling relations and implications for grain growth and radial drift

We analyse spatially resolved ALMA observations at 0.9, 1.3, and 3.1 mm for the 26 brightest protoplanetary discs in the Lupus star-forming region. We characterise the discs multi-wavelength brightness profiles by fitting the interferometric visibilities in a homogeneous way, obtaining effective disc sizes at the three wavelengths, spectral index profiles and optical depth estimates. We report three fundamental discoveries: first, the millimeter continuum size - luminosity relation already observed at 0.9 mm is also present at 1.3 mm with an identical slope, and at 3.1 mm with a steeper slope, confirming that emission at longer wavelengths becomes increasingly optically thin. Second, when observed at 3.1 mm the discs appear to be only 9% smaller than when observed at 0.9 mm, in tension with models of dust evolution which predict a starker difference. Third, by forward modelling the sample of measurements with a simple parametric disc model, we find that the presence of large grains ($a_\mathrm{max}>1 $mm) throughout the discs is the most favoured explanation for all discs as it reproduces simultaneously their spectral indices, optical depth, luminosity, and radial extent in the 0.9-1.3 mm wavelength range. We also find that the observations can be alternatively interpreted with the discs being dominated by optically thick, unresolved, substructures made of mm-sized grains with a high scattering albedo.

==> figures/fits/sample_clean/fit_results_latex_sample_clean.tex <==

\begin{table*}
 \caption{Parameters of the inferred brightness profiles: modified self-similar brightness.}
 \centering
 \resizebox{\textwidth}{!}{%
 \begin{tabular}{lccccccc|ccc}
   \midrule
   \toprule
Name & $\lambda$
 & $I_0$ & $R_c$ & $\gamma_1$ & $\gamma_2$
 & $i$ & $P.A.$
 & $F_\mathrm{tot}$ & $\rho_{68}$ & $R_{68}$ \\ 
 & (mm)
 & (Jy sr$^{-1}$) & ($\arcsec$) &  & 
 & $(^\circ)$ & $(^\circ)$
 & (mJy) & $(\arcsec)$ & (au) \\ 
   \midrule
Sz 65                & $0.89$
 & $10.63^{\pm0.32}$ & $0.18^{\pm0.05}$ & $-0.34^{\pm0.41}$ & $2.44^{\pm1.08}$
 & $56^{\pm1}$ & $109^{\pm1}$
 & $63.5^{\pm0.8}$ & $0.162^{\pm0.005}$ & $25.1^{\pm0.8}$ \\ 
                     & $1.33$
 & $10.12^{\pm0.11}$ & $0.22^{\pm0.02}$ & $-0.56^{\pm0.14}$ & $3.94^{\pm0.86}$
 & $61^{\pm1}$ & $113^{\pm1}$
 & $28.9^{\pm0.2}$ & $0.166^{\pm0.003}$ & $25.7^{\pm0.5}$ \\ 
                     & $3.10$
 & $8.93^{\pm0.53}$ & $0.24^{\pm0.09}$ & $-1.14^{\pm0.38}$ & $2.42^{\pm1.24}$
 & $47^{\pm6}$ & $100^{\pm7}$
 & $4.9^{\pm0.2}$ & $0.145^{\pm0.012}$ & $22.4^{\pm1.8}$ \\ 
Sz 71                & $0.89$
 & $9.95^{\pm0.05}$ & $0.53^{\pm0.02}$ & $-0.66^{\pm0.04}$ & $1.96^{\pm0.13}$
 & $42^{\pm1}$ & $38^{\pm1}$
 & $183.0^{\pm1.2}$ & $0.450^{\pm0.004}$ & $69.9^{\pm0.7}$ \\ 
                     & $1.33$
 & $9.69^{\pm0.06}$ & $0.45^{\pm0.03}$ & $-0.63^{\pm0.04}$ & $1.92^{\pm0.15}$
 & $40^{\pm1}$ & $27^{\pm1}$
 & $73.9^{\pm0.5}$ & $0.392^{\pm0.004}$ & $60.8^{\pm0.6}$ \\ 
                     & $3.10$
 & $9.37^{\pm0.31}$ & $0.21^{\pm0.10}$ & $-0.46^{\pm0.24}$ & $1.08^{\pm0.25}$
 & $39^{\pm3}$ & $29^{\pm4}$
 & $9.6^{\pm0.2}$ & $0.339^{\pm0.011}$ & $52.6^{\pm1.7}$ \\ 
Sz 82                & $0.90$
 & $9.27^{\pm0.00}$ & $1.96^{\pm0.00}$ & $-1.11^{\pm0.00}$ & $5.00^{\pm0.00}$
 & $52^{\pm0}$ & $144^{\pm0}$
 & $674.8^{\pm0.8}$ & $1.184^{\pm0.002}$ & $186.8^{\pm0.2}$ \\ 
                     & $1.28$
 & $8.70^{\pm0.01}$ & $1.67^{\pm0.03}$ & $-1.27^{\pm0.01}$ & $4.52^{\pm0.32}$
 & $33^{\pm1}$ & $0^{\pm0}$
 & $221.5^{\pm2.2}$ & $0.905^{\pm0.013}$ & $142.8^{\pm2.0}$ \\ 
                     & $3.10$
 & $12.13^{\pm0.05}$ & $0.00^{\pm0.00}$ & $-1.27^{\pm0.03}$ & $0.21^{\pm0.01}$
 & $26^{\pm1}$ & $0^{\pm0}$
 & $19.6^{\pm0.2}$ & $0.821^{\pm0.036}$ & $129.4^{\pm5.7}$ \\ 
Sz 83                & $0.89$
 & $10.46^{\pm0.05}$ & $0.39^{\pm0.01}$ & $-0.73^{\pm0.05}$ & $3.73^{\pm0.51}$
 & $22^{\pm1}$ & $89^{\pm4}$
 & $428.1^{\pm2.3}$ & $0.279^{\pm0.002}$ & $44.2^{\pm0.3}$ \\ 
                     & $1.33$
 & $10.03^{\pm0.02}$ & $0.39^{\pm0.00}$ & $-0.78^{\pm0.02}$ & $4.66^{\pm0.28}$
 & $22^{\pm1}$ & $125^{\pm3}$
 & $167.3^{\pm0.7}$ & $0.272^{\pm0.002}$ & $43.2^{\pm0.3}$ \\ 
                     & $3.11$
 & $9.12^{\pm0.03}$ & $0.36^{\pm0.01}$ & $-0.98^{\pm0.03}$ & $4.39^{\pm0.50}$
 & $17^{\pm2}$ & $112^{\pm7}$
 & $22.3^{\pm0.1}$ & $0.233^{\pm0.002}$ & $37.1^{\pm0.2}$ \\ 
Sz 84                & $0.89$
 & $10.77^{\pm0.14}$ & $0.15^{\pm0.07}$ & $0.99^{\pm0.71}$ & $1.65^{\pm0.58}$
 & $75^{\pm1}$ & $168^{\pm1}$
 & $32.6^{\pm0.6}$ & $0.241^{\pm0.006}$ & $36.6^{\pm0.9}$ \\ 
                     & $1.33$
 & $10.24^{\pm0.14}$ & $0.13^{\pm0.07}$ & $1.08^{\pm0.65}$ & $1.43^{\pm0.50}$
 & $69^{\pm1}$ & $170^{\pm1}$
 & $12.5^{\pm0.2}$ & $0.245^{\pm0.005}$ & $37.3^{\pm0.8}$ \\ 
                     & $3.10$
 & $8.87^{\pm0.33}$ & $0.28^{\pm0.07}$ & $0.19^{\pm0.88}$ & $3.35^{\pm1.16}$
 & $65^{\pm4}$ & $167^{\pm4}$
 & $1.5^{\pm0.0}$ & $0.253^{\pm0.018}$ & $38.5^{\pm2.8}$ \\ 
Sz 129               & $0.89$
 & $10.28^{\pm0.05}$ & $0.37^{\pm0.01}$ & $-0.39^{\pm0.06}$ & $3.08^{\pm0.29}$
 & $32^{\pm1}$ & $153^{\pm1}$
 & $179.6^{\pm0.8}$ & $0.298^{\pm0.002}$ & $47.9^{\pm0.3}$ \\ 
                     & $1.33$
 & $10.07^{\pm0.06}$ & $0.33^{\pm0.02}$ & $-0.17^{\pm0.08}$ & $2.32^{\pm0.21}$
 & $39^{\pm1}$ & $156^{\pm1}$
 & $75.5^{\pm0.5}$ & $0.313^{\pm0.003}$ & $50.4^{\pm0.4}$ \\ 
                     & $3.10$
 & $9.69^{\pm0.30}$ & $0.15^{\pm0.10}$ & $0.11^{\pm0.52}$ & $1.18^{\pm0.43}$
 & $40^{\pm2}$ & $147^{\pm3}$
 & $9.5^{\pm0.2}$ & $0.278^{\pm0.007}$ & $44.7^{\pm1.2}$ \\ 
J15592838-4021513    & $0.89$
 & $10.12^{\pm0.08}$ & $0.19^{\pm0.01}$ & $4.88^{\pm0.12}$ & $1.48^{\pm0.04}$
 & $68^{\pm0}$ & $109^{\pm0}$
 & $275.6^{\pm1.1}$ & $0.602^{\pm0.002}$ & $95.3^{\pm0.4}$ \\ 
                     & $1.33$
 & $10.23^{\pm0.06}$ & $0.33^{\pm0.03}$ & $3.13^{\pm0.28}$ & $1.89^{\pm0.13}$
 & $67^{\pm0}$ & $109^{\pm0}$
 & $87.3^{\pm0.4}$ & $0.606^{\pm0.003}$ & $96.0^{\pm0.4}$ \\ 
                     & $3.10$
 & $9.10^{\pm0.12}$ & $0.44^{\pm0.16}$ & $1.50^{\pm0.83}$ & $2.14^{\pm0.89}$
 & $68^{\pm1}$ & $109^{\pm1}$
 & $6.4^{\pm0.2}$ & $0.597^{\pm0.015}$ & $94.5^{\pm2.3}$ \\ 
J16000236-4222145    & $0.89$
 & $9.82^{\pm0.03}$ & $0.68^{\pm0.01}$ & $-0.58^{\pm0.03}$ & $3.76^{\pm0.38}$
 & $65^{\pm0}$ & $161^{\pm0}$
 & $119.4^{\pm0.9}$ & $0.508^{\pm0.003}$ & $83.0^{\pm0.6}$ \\ 
                     & $1.33$
 & $9.55^{\pm0.03}$ & $0.62^{\pm0.02}$ & $-0.52^{\pm0.04}$ & $3.47^{\pm0.35}$
 & $66^{\pm0}$ & $161^{\pm0}$
 & $49.5^{\pm0.4}$ & $0.479^{\pm0.005}$ & $78.3^{\pm0.9}$ \\ 
                     & $3.10$
 & $8.83^{\pm0.29}$ & $0.45^{\pm0.13}$ & $-0.40^{\pm0.32}$ & $2.09^{\pm0.88}$
 & $56^{\pm2}$ & $164^{\pm2}$
 & $6.5^{\pm0.2}$ & $0.410^{\pm0.011}$ & $67.0^{\pm1.8}$ \\ 
J16004452-4155310    & $0.89$
 & $10.63^{\pm0.08}$ & $0.44^{\pm0.03}$ & $-0.18^{\pm0.11}$ & $2.97^{\pm0.48}$
 & $73^{\pm0}$ & $59^{\pm0}$
 & $172.5^{\pm1.2}$ & $0.377^{\pm0.003}$ & $58.8^{\pm0.4}$ \\ 
                     & $1.33$
 & $10.46^{\pm0.11}$ & $0.26^{\pm0.05}$ & $0.39^{\pm0.23}$ & $1.59^{\pm0.23}$
 & $66^{\pm0}$ & $54^{\pm0}$
 & $66.8^{\pm0.5}$ & $0.375^{\pm0.003}$ & $58.5^{\pm0.5}$ \\ 
                     & $3.10$
 & $9.42^{\pm0.24}$ & $0.29^{\pm0.09}$ & $0.14^{\pm0.44}$ & $1.96^{\pm0.74}$
 & $59^{\pm1}$ & $54^{\pm1}$
 & $8.4^{\pm0.1}$ & $0.329^{\pm0.007}$ & $51.3^{\pm1.1}$ \\ 
J16011549-4152351    & $0.89$
 & $9.48^{\pm0.06}$ & $0.81^{\pm0.03}$ & $-0.82^{\pm0.04}$ & $2.85^{\pm0.52}$
 & $67^{\pm1}$ & $156^{\pm1}$
 & $86.9^{\pm1.7}$ & $0.576^{\pm0.015}$ & $92.2^{\pm2.3}$ \\ 
                     & $1.33$
 & $8.80^{\pm0.04}$ & $0.90^{\pm0.03}$ & $-0.98^{\pm0.02}$ & $3.17^{\pm0.49}$
 & $69^{\pm1}$ & $155^{\pm1}$
 & $23.7^{\pm0.4}$ & $0.587^{\pm0.010}$ & $94.0^{\pm1.6}$ \\ 
                     & $3.10$
 & $7.61^{\pm0.20}$ & $0.98^{\pm0.17}$ & $-1.11^{\pm0.10}$ & $2.80^{\pm1.32}$
 & $66^{\pm3}$ & $156^{\pm3}$
 & $2.5^{\pm0.2}$ & $0.623^{\pm0.063}$ & $99.6^{\pm10.0}$ \\ 
Sz 133               & $0.89$
 & $10.34^{\pm0.15}$ & $0.43^{\pm0.08}$ & $-0.18^{\pm0.16}$ & $1.88^{\pm0.38}$
 & $78^{\pm1}$ & $127^{\pm0}$
 & $69.7^{\pm1.1}$ & $0.456^{\pm0.009}$ & $70.5^{\pm1.4}$ \\ 
                     & $1.33$
 & $9.77^{\pm0.08}$ & $0.49^{\pm0.03}$ & $-0.36^{\pm0.10}$ & $3.02^{\pm0.55}$
 & $77^{\pm0}$ & $127^{\pm0}$
 & $26.6^{\pm0.2}$ & $0.403^{\pm0.006}$ & $62.3^{\pm0.9}$ \\ 
                     & $3.10$
 & $8.80^{\pm0.17}$ & $0.48^{\pm0.06}$ & $-0.58^{\pm0.17}$ & $3.41^{\pm1.15}$
 & $75^{\pm1}$ & $127^{\pm1}$
 & $3.6^{\pm0.1}$ & $0.365^{\pm0.011}$ & $56.4^{\pm1.7}$ \\ 
J16070854-3914075    & $0.89$
 & $10.39^{\pm0.05}$ & $0.27^{\pm0.09}$ & $1.48^{\pm0.44}$ & $1.36^{\pm0.23}$
 & $73^{\pm0}$ & $155^{\pm0}$
 & $89.5^{\pm1.3}$ & $0.617^{\pm0.012}$ & $108.9^{\pm2.1}$ \\ 
                     & $1.33$
 & $10.03^{\pm0.07}$ & $0.24^{\pm0.07}$ & $1.94^{\pm0.39}$ & $1.36^{\pm0.18}$
 & $73^{\pm0}$ & $154^{\pm0}$
 & $35.4^{\pm0.3}$ & $0.593^{\pm0.005}$ & $104.7^{\pm0.9}$ \\ 
                     & $3.10$
 & $9.11^{\pm0.22}$ & $0.24^{\pm0.09}$ & $2.39^{\pm0.67}$ & $1.46^{\pm0.31}$
 & $71^{\pm1}$ & $156^{\pm1}$
 & $4.9^{\pm0.1}$ & $0.555^{\pm0.009}$ & $98.2^{\pm1.6}$ \\ 
Sz 98                & $0.89$
 & $9.47^{\pm0.01}$ & $1.07^{\pm0.01}$ & $-0.80^{\pm0.01}$ & $4.86^{\pm0.15}$
 & $47^{\pm1}$ & $109^{\pm1}$
 & $258.2^{\pm2.0}$ & $0.730^{\pm0.006}$ & $113.6^{\pm0.9}$ \\ 
                     & $1.33$
 & $9.45^{\pm0.04}$ & $0.77^{\pm0.03}$ & $-0.55^{\pm0.03}$ & $1.96^{\pm0.12}$
 & $47^{\pm1}$ & $113^{\pm1}$
 & $107.1^{\pm0.5}$ & $0.690^{\pm0.005}$ & $107.3^{\pm0.8}$ \\ 
                     & $3.11$
 & $8.15^{\pm0.05}$ & $0.97^{\pm0.03}$ & $-1.01^{\pm0.03}$ & $3.59^{\pm0.67}$
 & $47^{\pm1}$ & $111^{\pm2}$
 & $12.5^{\pm0.2}$ & $0.624^{\pm0.012}$ & $97.0^{\pm1.9}$ \\ 
Sz 100               & $0.89$
 & $10.54^{\pm0.09}$ & $0.16^{\pm0.04}$ & $3.54^{\pm0.90}$ & $2.31^{\pm0.51}$
 & $46^{\pm1}$ & $63^{\pm1}$
 & $54.0^{\pm0.5}$ & $0.259^{\pm0.003}$ & $35.3^{\pm0.4}$ \\ 
                     & $1.33$
 & $10.24^{\pm0.04}$ & $0.20^{\pm0.03}$ & $3.72^{\pm0.73}$ & $3.45^{\pm0.61}$
 & $42^{\pm1}$ & $67^{\pm2}$
 & $22.0^{\pm0.2}$ & $0.245^{\pm0.003}$ & $33.5^{\pm0.4}$ \\ 
                     & $3.10$
 & $9.05^{\pm0.15}$ & $0.28^{\pm0.06}$ & $1.01^{\pm0.63}$ & $3.26^{\pm1.09}$
 & $41^{\pm3}$ & $72^{\pm4}$
 & $3.1^{\pm0.1}$ & $0.283^{\pm0.007}$ & $38.7^{\pm1.0}$ \\ 
J16083070-3828268    & $0.89$
 & $10.80^{\pm0.02}$ & $0.48^{\pm0.02}$ & $4.84^{\pm0.17}$ & $4.26^{\pm0.35}$
 & $73^{\pm0}$ & $107^{\pm0}$
 & $134.2^{\pm0.9}$ & $0.558^{\pm0.003}$ & $86.7^{\pm0.5}$ \\ 
                     & $1.33$
 & $10.29^{\pm0.01}$ & $0.48^{\pm0.01}$ & $4.91^{\pm0.10}$ & $4.82^{\pm0.18}$
 & $72^{\pm0}$ & $108^{\pm0}$
 & $38.3^{\pm0.2}$ & $0.539^{\pm0.002}$ & $83.8^{\pm0.3}$ \\ 
                     & $3.10$
 & $9.22^{\pm0.08}$ & $0.51^{\pm0.06}$ & $3.75^{\pm1.34}$ & $4.90^{\pm1.32}$
 & $71^{\pm1}$ & $108^{\pm1}$
 & $4.1^{\pm0.1}$ & $0.546^{\pm0.012}$ & $84.9^{\pm1.9}$ \\ 
Sz 111               & $0.89$
 & $10.60^{\pm0.03}$ & $0.28^{\pm0.01}$ & $4.90^{\pm0.11}$ & $2.46^{\pm0.08}$
 & $54^{\pm0}$ & $44^{\pm0}$
 & $177.9^{\pm0.8}$ & $0.448^{\pm0.002}$ & $70.6^{\pm0.3}$ \\ 
                     & $1.33$
 & $10.12^{\pm0.05}$ & $0.29^{\pm0.02}$ & $4.82^{\pm0.20}$ & $2.54^{\pm0.14}$
 & $54^{\pm0}$ & $44^{\pm0}$
 & $58.6^{\pm0.3}$ & $0.454^{\pm0.002}$ & $71.6^{\pm0.3}$ \\ 
                     & $3.10$
 & $9.03^{\pm0.09}$ & $0.46^{\pm0.07}$ & $1.69^{\pm0.60}$ & $3.55^{\pm0.96}$
 & $52^{\pm2}$ & $41^{\pm2}$
 & $5.8^{\pm0.1}$ & $0.480^{\pm0.012}$ & $75.7^{\pm1.9}$ \\ 
Sz 114               & $0.89$
 & $9.73^{\pm0.02}$ & $0.38^{\pm0.01}$ & $-0.96^{\pm0.02}$ & $4.55^{\pm0.39}$
 & $15^{\pm3}$ & $158^{\pm9}$
 & $99.3^{\pm0.5}$ & $0.247^{\pm0.002}$ & $39.9^{\pm0.4}$ \\ 
                     & $1.33$
 & $9.59^{\pm0.08}$ & $0.34^{\pm0.02}$ & $-0.78^{\pm0.07}$ & $2.90^{\pm0.47}$
 & $30^{\pm2}$ & $0^{\pm0}$
 & $42.6^{\pm0.3}$ & $0.247^{\pm0.003}$ & $39.9^{\pm0.5}$ \\ 
                     & $3.10$
 & $8.46^{\pm0.22}$ & $0.37^{\pm0.06}$ & $-1.04^{\pm0.16}$ & $3.02^{\pm1.28}$
 & $11^{\pm8}$ & $82^{\pm64}$
 & $5.3^{\pm0.1}$ & $0.235^{\pm0.010}$ & $37.9^{\pm1.7}$ \\ 
Sz 118               & $0.89$
 & $10.58^{\pm0.05}$ & $0.32^{\pm0.05}$ & $3.23^{\pm0.80}$ & $3.61^{\pm0.90}$
 & $66^{\pm1}$ & $174^{\pm1}$
 & $60.8^{\pm0.7}$ & $0.369^{\pm0.005}$ & $60.3^{\pm0.8}$ \\ 
                     & $1.33$
 & $10.19^{\pm0.03}$ & $0.34^{\pm0.03}$ & $3.19^{\pm0.56}$ & $4.04^{\pm0.70}$
 & $66^{\pm0}$ & $172^{\pm0}$
 & $23.8^{\pm0.2}$ & $0.371^{\pm0.004}$ & $60.6^{\pm0.6}$ \\ 
                     & $3.10$
 & $9.11^{\pm0.07}$ & $0.28^{\pm0.08}$ & $2.34^{\pm0.87}$ & $2.33^{\pm0.88}$
 & $65^{\pm1}$ & $172^{\pm1}$
 & $2.9^{\pm0.1}$ & $0.395^{\pm0.012}$ & $64.4^{\pm1.9}$ \\ 
Sz 123               & $0.89$
 & $10.60^{\pm0.04}$ & $0.23^{\pm0.02}$ & $4.01^{\pm0.66}$ & $4.33^{\pm0.59}$
 & $51^{\pm1}$ & $154^{\pm1}$
 & $41.5^{\pm0.4}$ & $0.254^{\pm0.003}$ & $41.1^{\pm0.4}$ \\ 
                     & $1.33$
 & $10.21^{\pm0.03}$ & $0.23^{\pm0.02}$ & $3.87^{\pm0.67}$ & $4.36^{\pm0.57}$
 & $51^{\pm1}$ & $155^{\pm1}$
 & $16.1^{\pm0.1}$ & $0.251^{\pm0.003}$ & $40.7^{\pm0.4}$ \\ 
                     & $3.08$
 & $9.45^{\pm0.04}$ & $0.23^{\pm0.01}$ & $4.36^{\pm0.56}$ & $4.51^{\pm0.45}$
 & $56^{\pm1}$ & $155^{\pm1}$
 & $2.4^{\pm0.0}$ & $0.255^{\pm0.004}$ & $41.2^{\pm0.6}$ \\   \bottomrule
 \end{tabular}
  }
 \begin{flushleft}
 \textbf{Note}
 The parameter values are the medians of their posterior distributions, and the uncertainties represent the 68\% confidence interval. 
 The $F_\nu$ posterior does not include systematic flux calibration uncertainty. Note that the parameters to the right of the vertical bar ($F_\nu$, $\rhose$, $\Rse$) are not free parameters in the fit, but they are rather inferred from the joint posterior on $\left\{I_0,\ R_c,\ \gamma_1,\ \gamma_2\right\}$. 
 \end{flushleft}
\label{tb:fit.results.ss2s}
\end{table*}



==> figures/fits/sample_clean/latex_sample_clean.tex <==

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_65_images.pdf}
\caption{
Synthesized images of the Sz 65 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_65}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_65_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 65 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 1.125e+10 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_65}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_65_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 65 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_65}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_71_images.pdf}
\caption{
Synthesized images of the Sz 71 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_71}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_71_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 71 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 2.445e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_71}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_71_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 71 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_71}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_82_images.pdf}
\caption{
Synthesized images of the Sz 82 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_82}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_82_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 82 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 1.029e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_82}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_82_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 82 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_82}
\end{figure}

\clearpage

% Sz 83 is already present in the main text.
% \begin{figure}
% \centering
% \includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_83_images.pdf}
% \caption{
% Synthesized images of the Sz 83 observations (left), model (center), and residuals (right) at the three observing wavelengths.
% The model and residual images are the synthesized from the visibilities of the bestfit model. 
% The color scale is the same on each row.
% Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
% The synthesized beam is shown as a grey ellipse in each panel.
% }
% \label{fig:fits.images.Sz_83}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_83_brightness.pdf}
% \caption{ 
% \textit{Top}
% Brightness profile of Sz 83 at the three observing wavelengths.
% The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 1.180e+10 Jy/sr.
% \textit{Bottom}
% Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
% }
% \label{fig:fit.brightness.images.Sz_83}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_83_uvplot.pdf}
% \caption{
% Real part of the visibilities of Sz 83 as a function of deprojected baseline at the three observing wavelengths. 
% Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
% }
% \label{fig:fits.uvplot.Sz_83}
% \end{figure}

% \clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_84_images.pdf}
\caption{
Synthesized images of the Sz 84 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_84}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_84_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 84 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 3.102e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_84}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_84_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 84 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_84}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_129_images.pdf}
\caption{
Synthesized images of the Sz 129 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_129}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_129_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 129 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 4.951e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_129}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_129_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 129 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_129}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J15592838-4021513_images.pdf}
\caption{
Synthesized images of the J15592838-4021513 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.J15592838-4021513}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J15592838-4021513_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of J15592838-4021513 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 4.811e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.J15592838-4021513}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J15592838-4021513_uvplot.pdf}
\caption{
Real part of the visibilities of J15592838-4021513 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.J15592838-4021513}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J16000236-4222145_images.pdf}
\caption{
Synthesized images of the J16000236-4222145 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.J16000236-4222145}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J16000236-4222145_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of J16000236-4222145 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 2.748e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.J16000236-4222145}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J16000236-4222145_uvplot.pdf}
\caption{
Real part of the visibilities of J16000236-4222145 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.J16000236-4222145}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J16004452-4155310_images.pdf}
\caption{
Synthesized images of the J16004452-4155310 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.J16004452-4155310}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J16004452-4155310_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of J16004452-4155310 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 5.741e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.J16004452-4155310}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J16004452-4155310_uvplot.pdf}
\caption{
Real part of the visibilities of J16004452-4155310 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.J16004452-4155310}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J16011549-4152351_images.pdf}
\caption{
Synthesized images of the J16011549-4152351 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.J16011549-4152351}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J16011549-4152351_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of J16011549-4152351 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 7.424e+08 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.J16011549-4152351}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J16011549-4152351_uvplot.pdf}
\caption{
Real part of the visibilities of J16011549-4152351 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.J16011549-4152351}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_133_images.pdf}
\caption{
Synthesized images of the Sz 133 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_133}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_133_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 133 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 3.689e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_133}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_133_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 133 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_133}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J16070854-3914075_images.pdf}
\caption{
Synthesized images of the J16070854-3914075 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.J16070854-3914075}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J16070854-3914075_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of J16070854-3914075 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 2.025e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.J16070854-3914075}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J16070854-3914075_uvplot.pdf}
\caption{
Real part of the visibilities of J16070854-3914075 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.J16070854-3914075}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_98_images.pdf}
\caption{
Synthesized images of the Sz 98 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_98}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_98_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 98 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 1.348e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_98}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_98_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 98 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_98}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_100_images.pdf}
\caption{
Synthesized images of the Sz 100 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_100}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_100_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 100 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 5.378e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_100}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_100_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 100 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_100}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J16083070-3828268_images.pdf}
\caption{
Synthesized images of the J16083070-3828268 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.J16083070-3828268}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J16083070-3828268_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of J16083070-3828268 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 6.101e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.J16083070-3828268}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_J16083070-3828268_uvplot.pdf}
\caption{
Real part of the visibilities of J16083070-3828268 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.J16083070-3828268}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_111_images.pdf}
\caption{
Synthesized images of the Sz 111 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_111}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_111_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 111 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 5.021e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_111}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_111_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 111 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_111}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_114_images.pdf}
\caption{
Synthesized images of the Sz 114 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_114}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_114_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 114 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 3.389e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_114}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_114_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 114 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_114}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_118_images.pdf}
\caption{
Synthesized images of the Sz 118 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_118}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_118_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 118 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 4.875e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_118}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_118_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 118 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_118}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_123_images.pdf}
\caption{
Synthesized images of the Sz 123 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_123}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_123_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 123 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 5.079e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_123}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_clean/Multiw_Sz_123_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 123 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_123}
\end{figure}

\clearpage


==> figures/fits/sample_clean/tb_YSOs_sample_clean.tex <==

\begin{table*}
 \caption{Sample of young stellar objects in the Lupus region with ALMA observations at 0.9, 1.3, and 3.1 mm.}
 \centering
 %\resizebox{\textwidth}{!}{%
 \begin{tabular}{lllllcccl}
   \midrule
   \toprule
Name
 & R.A. & Dec.
 & 2MASS identifier & Gaia DR2 identifier
 & $d$ & $L_{\star}$ & Notes \\ 

 & (J2015.5) & (J2015.5)
 &  & 
 & (pc) & ($L_\odot$) &  \\ 
   \midrule
Sz 65               
 & 15:39:27.755   & -34:46:17.5538
 & J15392776-3446171    &  6013399894569703040
 & $154.6$ & $0.83$
 &  \\ 
Sz 66               
 & 15:39:28.2664  & -34:46:18.4208
 & J15392828-3446180    &  6013399830146943104
 & $156.7$ & $0.22$
 &  \\ 
J15450634-3417378   
 & 15:45:06.343   & -34:17:37.83  
 & J15450634-3417378    &                   -1
 & $160.0$ & ... & $^{(1)}$ \\ 
J15450887-3417333   
 & 15:45:08.8553  & -34:17:33.799 
 & J15450887-3417333    &  6014696875913435520
 & $154.6$ & $0.06$
 &  \\ 
Sz 69               
 & 15:45:17.3931  & -34:18:28.6363
 & J15451741-3418283    &  6014696635395266304
 & $153.9$ & $0.09$
 &  \\ 
Sz 71               
 & 15:46:44.7117  & -34:30:36.0393
 & J15464473-3430354    &  6014722194741392512
 & $155.2$ & $0.33$
 & $^{(2)}$ \\ 
Sz 72               
 & 15:47:50.611   & -35:28:35.7635
 & J15475062-3528353    &  6011573266459331072
 & $155.2$ & $0.27$
 &  \\ 
Sz 73               
 & 15:47:56.9254  & -35:14:35.1429
 & J15475693-3514346    &  6011593641784262400
 & $156.1$ & $0.46$
 &  \\ 
Sz 82               
 & 15:56:09.1909  & -37:56:06.4938
 & J15560921-3756057    &  6010135758090335232
 & $157.7$ & $2.60$
 & $^{(2)}$ \\ 
Sz 83               
 & 15:56:42.2959  & -37:49:15.8336
 & J15564230-3749154    &  6010114558131195392
 & $158.9$ & $1.49$
 & $^{(2)}$ \\ 
Sz 84               
 & 15:58:02.504   & -37:36:03.0868
 & J15580252-3736026    &  6010216537834709760
 & $152.0$ & $0.13$
 &  \\ 
Sz 129              
 & 15:59:16.4569  & -41:57:10.6586
 & J15591647-4157102    &  5995168724780802944
 & $160.9$ & $0.43$
 & $^{(2)}$ \\ 
J15592838-4021513   
 & 15:59:28.3716  & -40:21:51.5941
 & J15592838-4021513    &  5996151172781298304
 & $158.4$ & $1.87$
 &  \\ 
J16000236-4222145   
 & 16:00:02.3423  & -42:22:14.96  
 & J16000236-4222145    &  5995139484643284864
 & $163.4$ & $0.18$
 &  \\ 
J16004452-4155310   
 & 16:00:44.5041  & -41:55:31.2943
 & J16004452-4155310    &  5995177933191206016
 & $155.9$ & $0.85$
 & $^{(2)}$ \\ 
J16011549-4152351   
 & 16:01:15.492   & -41:52:35.19  
 & J16011549-4152351    &                   -1
 & $160.0$ & ... & $^{(1)}$ \\ 
Sz 133              
 & 16:03:29.3745  & -41:40:02.1686
 & J16032939-4140018    &  5995094095435598848
 & $154.6$ & $0.07$
 &  \\ 
J16070854-3914075   
 & 16:07:08.538   & -39:14:07.8853
 & J16070854-3914075    &  5997076721058575360
 & $176.7$ & $0.14$
 &  \\ 
Sz 90               
 & 16:07:10.057   & -39:11:03.6527
 & J16071007-3911033    &  5997077167735183872
 & $159.7$ & $0.42$
 &  \\ 
Sz 98               
 & 16:08:22.4807  & -39:04:46.8072
 & J16082249-3904464    &  5997082867132347136
 & $155.5$ & $1.53$
 &  \\ 
Sz 100              
 & 16:08:25.7497  & -39:06:01.5904
 & J16082576-3906011    &  5997082046818385408
 & $136.5$ & $0.08$
 &  \\ 
J16083070-3828268   
 & 16:08:30.6864  & -38:28:27.2382
 & J16083070-3828268    &  5997490206145065088
 & $155.4$ & $1.84$
 &  \\ 
Sz 108B             
 & 16:08:42.8697  & -39:06:15.0303
 & -3                   &  5997082218616859264
 & $168.3$ & $0.11$
 &  \\ 
Sz 110              
 & 16:08:51.5567  & -39:03:18.0683
 & J16085157-3903177    &  5997082390415552768
 & $158.8$ & $0.18$
 &  \\ 
J16085324-3914401   
 & 16:08:53.2281  & -39:14:40.5292
 & J16085324-3914401    &  5997033290348155136
 & $167.0$ & $0.21$
 &  \\ 
Sz 111              
 & 16:08:54.6719  & -39:37:43.4964
 & J16085468-3937431    &  5997006897751436544
 & $157.6$ & $0.21$
 &  \\ 
Sz 113              
 & 16:08:57.7897  & -39:02:23.2136
 & J16085780-3902227    &  5997457736191421184
 & $162.5$ & $0.04$
 &  \\ 
Sz 114              
 & 16:09:01.836   & -39:05:12.7872
 & J16090185-3905124    &  5997410491550194816
 & $161.5$ & $0.21$
 & $^{(2)}$ \\ 
Sz 118              
 & 16:09:48.6421  & -39:11:17.2127
 & J16094864-3911169    &  5997405509388068352
 & $163.1$ & $0.72$
 &  \\ 
Sz 123              
 & 16:10:51.5731  & -38:53:14.1302
 & J16105158-3853137    &  5997416573223873536
 & $162.1$ & $0.13$
 &  \\ 
J16124373-3815031   
 & 16:12:43.7388  & -38:15:03.4229
 & J16124373-3815031    &  5997549820286701440
 & $159.1$ & $0.39$
 &  \\   \bottomrule
 \end{tabular}
  %}
 \begin{flushleft}
 \textbf{Note.}
 Name is the designation used in this paper (with notable alternative names where available).
 Right Ascension (R.A.) and Declination (Dec.) are from Gaia DR2 \citep{Gaia-Collaboration:2018aa}. 
 Distances ($d$) are computed using Gaia DR2 data by \cite{Bailer-Jones:2018aa}. 
 % Stellar masses ($M_\star$) are computed by \cite{Ansdell:2016qf} using \cite{Siess:2000qy} evolutionary tracks.
 Stellar bolometric luminosities ($L_\star$) are measured by \cite{Alcala:2017aa} from spectroscopic observations and corrected for Gaia DR2 distances by \cite{Alcala:2019aa}.
$^{(1)}$~Not found in Gaia DR2. For this source, we assume the average distance of the Lupus cloud complex (160 pc, \citealt{Manara:2018aa}). $^{(2)}$~Observed in the DSHARP survey \citep{Andrews:2018aa}.
\end{flushleft}
\label{tb:YSOs}
\end{table*}



==> figures/fits/sample_noisy/.ipynb_checkpoints/fit_results_latex_sample_noisy-checkpoint.tex <==

\begin{table*}
 \caption{Parameters of the inferred brightness profiles: Gaussian brightness.}
 \centering
 \begin{tabular}{lccccc|ccc}
   \midrule
   \toprule
Name & $\lambda$
 & $F_\mathrm{\nu}$ & $\sigma$ & $i$ & $P.A.$
 & $\rho_{68}$ & $R_{68}$ \\ 
 & (mm)
 & (mJy) & ($\arcsec$) & $(^\circ)$ & $(^\circ)$
 & $(\arcsec)$ & (au) \\ 
   \midrule
J15450887-3417333    & $0.89$
 & $42.9^{\pm0.6}$ & $0.08^{\pm0.00}$ & $35^{\pm5}$ & $64^{\pm8}$
 & $0.122^{\pm0.005}$ & $18.9^{\pm0.8}$ \\ 
                     & $1.33$
 & $19.8^{\pm0.2}$ & $0.10^{\pm0.00}$ & $59^{\pm1}$ & $174^{\pm2}$
 & $0.149^{\pm0.003}$ & $23.1^{\pm0.4}$ \\ 
                     & $3.10$
 & $3.7^{\pm0.1}$ & $0.07^{\pm0.01}$ & $42^{\pm10}$ & $160^{\pm15}$
 & $0.110^{\pm0.012}$ & $16.9^{\pm1.9}$ \\ 
Sz 69                & $0.89$
 & $14.8^{\pm5.1}$ & $0.04^{\pm0.00}$ & $68^{\pm16}$ & $165^{\pm9}$
 & $0.068^{\pm0.006}$ & $10.4^{\pm1.0}$ \\ 
                     & $1.33$
 & $7.6^{\pm0.2}$ & $0.05^{\pm0.00}$ & $51^{\pm9}$ & $134^{\pm10}$
 & $0.075^{\pm0.007}$ & $11.5^{\pm1.0}$ \\ 
                     & $3.08$
 & $1.5^{\pm0.1}$ & $0.03^{\pm0.01}$ & $47^{\pm22}$ & $96^{\pm26}$
 & $0.050^{\pm0.009}$ & $7.6^{\pm1.4}$ \\ 
Sz 72                & $0.89$
 & $13.9^{\pm0.2}$ & $0.05^{\pm0.00}$ & $46^{\pm16}$ & $34^{\pm16}$
 & $0.083^{\pm0.008}$ & $12.8^{\pm1.2}$ \\ 
                     & $1.33$
 & $5.7^{\pm0.1}$ & $0.05^{\pm0.00}$ & $24^{\pm15}$ & $140^{\pm74}$
 & $0.081^{\pm0.005}$ & $12.6^{\pm0.8}$ \\ 
                     & $3.08$
 & $0.9^{\pm0.0}$ & $0.04^{\pm0.01}$ & $49^{\pm29}$ & $45^{\pm46}$
 & $0.063^{\pm0.012}$ & $9.7^{\pm1.9}$ \\ 
Sz 90                & $0.89$
 & $21.8^{\pm0.4}$ & $0.08^{\pm0.00}$ & $59^{\pm6}$ & $124^{\pm5}$
 & $0.125^{\pm0.006}$ & $19.9^{\pm1.0}$ \\ 
                     & $1.33$
 & $8.7^{\pm0.1}$ & $0.10^{\pm0.00}$ & $57^{\pm3}$ & $141^{\pm3}$
 & $0.146^{\pm0.005}$ & $23.4^{\pm0.7}$ \\ 
                     & $3.10$
 & $1.1^{\pm0.0}$ & $0.09^{\pm0.01}$ & $55^{\pm11}$ & $140^{\pm10}$
 & $0.140^{\pm0.021}$ & $22.3^{\pm3.3}$ \\ 
Sz 108B              & $0.89$
 & $26.9^{\pm0.6}$ & $0.10^{\pm0.00}$ & $46^{\pm5}$ & $151^{\pm6}$
 & $0.151^{\pm0.006}$ & $25.5^{\pm1.0}$ \\ 
                     & $1.33$
 & $11.9^{\pm0.2}$ & $0.10^{\pm0.00}$ & $48^{\pm2}$ & $143^{\pm3}$
 & $0.154^{\pm0.004}$ & $25.9^{\pm0.7}$ \\ 
                     & $3.10$
 & $1.6^{\pm0.0}$ & $0.10^{\pm0.01}$ & $53^{\pm7}$ & $4^{\pm4}$
 & $0.154^{\pm0.012}$ & $25.9^{\pm2.0}$ \\ 
J16085324-3914401    & $0.89$
 & $19.9^{\pm0.4}$ & $0.06^{\pm0.01}$ & $50^{\pm8}$ & $99^{\pm11}$
 & $0.083^{\pm0.009}$ & $13.8^{\pm1.5}$ \\ 
                     & $1.33$
 & $7.6^{\pm0.1}$ & $0.07^{\pm0.00}$ & $54^{\pm5}$ & $131^{\pm5}$
 & $0.101^{\pm0.005}$ & $16.8^{\pm0.9}$ \\ 
                     & $3.10$
 & $1.4^{\pm0.0}$ & $0.06^{\pm0.01}$ & $29^{\pm20}$ & $96^{\pm38}$
 & $0.089^{\pm0.010}$ & $14.9^{\pm1.7}$ \\ 
J16124373-3815031    & $0.89$
 & $29.6^{\pm0.5}$ & $0.07^{\pm0.00}$ & $43^{\pm7}$ & $22^{\pm10}$
 & $0.105^{\pm0.006}$ & $16.7^{\pm1.0}$ \\ 
                     & $1.33$
 & $11.5^{\pm0.1}$ & $0.09^{\pm0.00}$ & $51^{\pm2}$ & $179^{\pm1}$
 & $0.131^{\pm0.003}$ & $20.8^{\pm0.5}$ \\ 
                     & $3.10$
 & $1.8^{\pm0.0}$ & $0.07^{\pm0.01}$ & $55^{\pm14}$ & $20^{\pm83}$
 & $0.104^{\pm0.016}$ & $16.5^{\pm2.5}$ \\   \bottomrule
 \end{tabular}
 \begin{flushleft}
 \textbf{Note}
 The parameter values are the medians of their posterior distributions, and the uncertainties represent the 68\% confidence interval. 
 The $F_\nu$ posterior does not include systematic flux calibration uncertainty. Note that the parameters to the right of the vertical bar ($\rhose$, $\Rse$) are not free parameters in the fit, but they are rather inferred from the joint posterior on $\left\{F_\nu,\ \sigma\right\}$. 
 \end{flushleft}
\label{tb:fit.results.gaussian}
\end{table*}



==> figures/fits/sample_noisy/latex_sample_noisy.tex <==
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_J15450887-3417333_images.pdf}
\caption{
Synthesized images of the J15450887-3417333 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.J15450887-3417333}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_J15450887-3417333_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of J15450887-3417333 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 8.494e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.J15450887-3417333}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_J15450887-3417333_uvplot.pdf}
\caption{
Real part of the visibilities of J15450887-3417333 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.J15450887-3417333}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_Sz_69_images.pdf}
\caption{
Synthesized images of the Sz 69 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_69}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_Sz_69_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 69 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 9.984e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_69}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_Sz_69_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 69 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_69}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_Sz_72_images.pdf}
\caption{
Synthesized images of the Sz 72 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_72}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_Sz_72_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 72 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 4.711e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_72}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_Sz_72_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 72 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_72}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_Sz_90_images.pdf}
\caption{
Synthesized images of the Sz 90 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_90}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_Sz_90_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 90 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 3.620e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_90}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_Sz_90_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 90 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_90}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_Sz_108B_images.pdf}
\caption{
Synthesized images of the Sz 108B observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.Sz_108B}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_Sz_108B_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of Sz 108B at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 3.653e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.Sz_108B}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_Sz_108B_uvplot.pdf}
\caption{
Real part of the visibilities of Sz 108B as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.Sz_108B}
\end{figure}

\clearpage


\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_J16085324-3914401_images.pdf}
\caption{
Synthesized images of the J16085324-3914401 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.J16085324-3914401}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_J16085324-3914401_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of J16085324-3914401 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 6.270e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.J16085324-3914401}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_J16085324-3914401_uvplot.pdf}
\caption{
Real part of the visibilities of J16085324-3914401 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.J16085324-3914401}
\end{figure}

\clearpage

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_J16124373-3815031_images.pdf}
\caption{
Synthesized images of the J16124373-3815031 observations (left), model (center), and residuals (right) at the three observing wavelengths.
The model and residual images are the synthesized from the visibilities of the bestfit model. 
The color scale is the same on each row.
Contours in the residuals are drawn at -3, 3, 6, 12, 24, etc. times the rms noise. 
The synthesized beam is shown as a grey ellipse in each panel.
}
\label{fig:fits.images.J16124373-3815031}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_J16124373-3815031_brightness.pdf}
\caption{ 
\textit{Top}
Brightness profile of J16124373-3815031 at the three observing wavelengths.
The profiles have been normalised to the brightness emitted at 1.3 mm at the radius enclosing 68\% of the 1.3 mm emission: 5.282e+09 Jy/sr.
\textit{Bottom}
Spectral index profile between 3.1 mm and 0.9 mm (yellow dashed) and between 3.1 mm and 1.3 mm (red dashed).
}
\label{fig:fit.brightness.images.J16124373-3815031}
\end{figure}
 
\begin{figure}
\centering
\includegraphics[width=\hsize]{figures/fits/sample_noisy/Multiw_J16124373-3815031_uvplot.pdf}
\caption{
Real part of the visibilities of J16124373-3815031 as a function of deprojected baseline at the three observing wavelengths. 
Data (filled circles) have been deprojected using $i$, $PA$ of the bestfit model (solid lines) and binned every 15k$\lambda$.
}
\label{fig:fits.uvplot.J16124373-3815031}
\end{figure}


==> sample_clean_analysis/latex_sample_clean_analysis.tex <==

\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/R68_vs_freq_sample_clean_slopes.pdf}
\caption{Caption}
\label{fig:R68_vs_freq_sample_clean_slopes}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/Ftot_vs_R68_sample_clean_unnormalised_narrow.pdf}
\caption{Caption}
\label{fig:Ftot_vs_R68_sample_clean_unnormalised_narrow}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/R68_vs_Ftot_split_panels_sample_cleanregression_clean.pdf}
\caption{Caption}
\label{fig:R68_vs_Ftot_split_panels_sample_cleanregression_clean}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/R68_vs_Ftot_split_panels_sample_clean.pdf}
\caption{Caption}
\label{fig:R68_vs_Ftot_split_panels_sample_clean}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/R68_vs_Lmm3mm_sample_clean_.pdf}
\caption{Caption}
\label{fig:R68_vs_Lmm3mm_sample_clean_}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/R68_vs_freq_sample_clean_normB7_with_median_slopes.pdf}
\caption{Caption}
\label{fig:R68_vs_freq_sample_clean_normB7_with_median_slopes}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/alphaB36_histogram_sample_clean.pdf}
\caption{Caption}
\label{fig:alphaB36_histogram_sample_clean}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/R68_vs_Ftot_split_panels_sample_cleanregression_joint_larger_uncertainty_noisy.pdf}
\caption{Caption}
\label{fig:R68_vs_Ftot_split_panels_sample_cleanregression_joint_larger_uncertainty_noisy}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/ff_vs_R68_sample_clean.pdf}
\caption{Caption}
\label{fig:ff_vs_R68_sample_clean}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/radii_slopes_hist_sample_clean.pdf}
\caption{Caption}
\label{fig:radii_slopes_hist_sample_clean}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/alpha_vs_R68_sample_clean_unnormalised_RB3_narrow.pdf}
\caption{Caption}
\label{fig:alpha_vs_R68_sample_clean_unnormalised_RB3_narrow}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/R68_vs_freq_sample_clean_slopes_unnormalised_Lupus_only.pdf}
\caption{Caption}
\label{fig:R68_vs_freq_sample_clean_slopes_unnormalised_Lupus_only}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/R68_vs_Ftot_sample_clean.pdf}
\caption{Caption}
\label{fig:R68_vs_Ftot_sample_clean}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/radii_ratios_histogram_sample_clean.pdf}
\caption{Caption}
\label{fig:radii_ratios_histogram_sample_clean}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/R68_vs_Ftot_sample_clean_normB7.pdf}
\caption{Caption}
\label{fig:R68_vs_Ftot_sample_clean_normB7}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/R68_vs_Ftot_sample_clean_normB6.pdf}
\caption{Caption}
\label{fig:R68_vs_Ftot_sample_clean_normB6}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/alpha37_vs_R68ratios_sample_clean_.pdf}
\caption{Caption}
\label{fig:alpha37_vs_R68ratios_sample_clean_}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/ff_vs_Ftot_sample_clean.pdf}
\caption{Caption}
\label{fig:ff_vs_Ftot_sample_clean}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=\hsize]{sample_clean_analysis/R68_vs_freq_sample_clean_slopes_unnormalised.pdf}
\caption{Caption}
\label{fig:R68_vs_freq_sample_clean_slopes_unnormalised}
\end{figure}


